Reconfigurable routing in data center networks

A hybrid network is a static (electronic) network that is augmented with optical switches. The Reconfigurable Routing Problem (RRP) in hybrid networks is the problem of finding settings for the optical switches augmenting a static network so as to achieve optimal delivery of some given workload. The problem has previously been studied in various scenarios with both tractability and NP-hardness results obtained. However, the data center and interconnection networks to which the problem is most relevant are almost always such that the static network is highly structured (and often node-symmetric) whereas all previous results assume that the static network can be arbitrary (which makes existing computational hardness results less technologically relevant and also easier to obtain). In this paper, and for the first time, we prove various intractability results for RRP where the underlying static network is highly structured, for example consisting of a hypercube, and also extend some existing tractability results.

==> lunar-section.tex <==
\section{The case of $\delta=1$}

This section is devoted to the restriction of RRP where the dynamic link limit $\delta$ is set to 1 - where any flow-path must use no more than a single dynamic link. We shall require substantially different techniques from those we have used in the remainder of this work to prove our main result, which entails that the problem \textsc{1-switched RRP}($\sigma=1$) is NP-complete for various graph classes including hypercubes, grids and toroidal grids. 
The intention is that this section provides a convenient template for proving hardness of the problem for other practically interesting classes beyond these. 


\subsection{Additional Definitions}

We begin with some basic definitions from graph theory. Let $G=(V,E)$ be a simple undirected graph. 
We define the \emph{open neighborhood} of a vertex $v$ to be $N(v):=\{u : (u,v) \in E\}$, and its closed neighborhood $N[v]:=N(v) \cup \{v\}$. Likewise for any set of vertices $S$, we define $N[S]:=\cup_{v \in S} N[v]$ and $N(S):=N[V] \setminus S$. 
A \emph{dominating set} in $G$ is a set of vertices $s$ such that each vertex in $G$ is either in $S$ or adjacent to a vertex in $S$. The \emph{domination number} of $G$, denoted $\gamma(G)$, is the least number of vertices in any dominating set of $G$. \textsc{Dominating Set} is the decision problem asking, for input $G$ and $k$, whether $\gamma(G) \le k$.

Where $S \subseteq V$ is a set of vertices in the graph, we denote $G[S]$ the subgraph of $G$ induced by $S$. That is, $G[S]$ has $S$ as its set of vertices and as edges exactly those edges of $G$ with both endpoints incident to a vertex in $S$. Also, $\mathrm{dist}_G(u,v)$ is the number of edges on the shortest path between $u$ and $v$ in $G$. %We call a shortest path between $u$ and $v$ a $u-v$ \emph{geodesic}.

\begin{definition}[Ball, Sphere]
    Where $G$ is a graph, we denote $B_G(v,r)$ (resp. $S_G(v,r)$) the \emph{ball} (resp. \emph{sphere}) with center $v$ and radius $r$ in $G$. Formally these are sets of vertices defined as:
    \begin{align*}
        B_G(v,r) &:= \{u : \mathrm{dist}_G(u,v) \le r\} \\
        S_G(v,r) &:= \{u : \mathrm{dist}_G(u,v) = r\} 
    \end{align*}
    % \red{[Unsure if needed -]}
    % Accordingly, where $T$ is a set of vertices in $G$ we define the ball $B(T,r)$ to be the union of all balls with center $t \in T$ and radius $r$ (i.e. all nodes at distance at most $r$ from some node $t \in T$). The sphere $S(T,r)=B(T,r) \setminus B(T,r-1)$ (note that we obtain the natural property that $S(T,1)=N(T)$).
\end{definition}


\noindent We shall also make use of the following (likely non-standard) definitions.

\begin{definition}[Restriction of decision problems to a graph class]
    Let $\Pi$ be a decision problem which takes one or many inputs, exactly one of which is a simple undirected graph. We denote $\Pi(\mathcal{G})$ the restriction of $\Pi$ to the graph class $\mathcal{G}$. That is, $\Pi(\mathcal{G})$ has as yes-instances exactly those yes-instances of $\Pi$ where the graph portion of the input also belongs to $\mathcal{G}$.
\end{definition}

We introduce a new graph problem, which is subtly different from the classic \textsc{Dominating Set}.

\begin{framed}
    \noindent
    \textbf{\textsc{Partial Domination}}\\
    \emph{Input:} Simple undirected graph $G=(V,E)$; set $T \subseteq V$; integer $k$.\\
    \emph{Question:} Is $(G[T],k)$ a yes-instance of \textsc{Dominating Set}? Equivalently, is there some set $X\subseteq T$ with $|X| \le k$ such that $T \subseteq N[X]$?
\end{framed}

% For natural graph classes, we would expect that if \textsc{Dominating Set}$(\mathcal{G})$ is NP-complete, then \textsc{Partial Domination}$(\mathcal{G})$ is NP-complete.
% \red{What if $\mathcal{G}$ is very hard to produce witness structures for? Possible diversion for IPL letter, not for here.} The problem of deciding whether a graph $G$ is an induced subgraph of a grid is NP-complete . 


\subsection{Hardness of \textsc{Partial Domination} on grids and hypercubes}

This subsection leverages several results from the literature, which more or less straightforwardly yield the desired results. 

\begin{theorem}[\cite{CCJ90} Theorem 5.1]
    \textsc{Dominating Set}(Induced subgraphs of grids) is NP-complete.
\end{theorem}

Note that the corollary below relies on some subtle properties of the proof applied in \cite{CCJ90} (namely, that the construction described explicitly describes an embedding into some grid). 
It is in general NP-hard, given some graph, to determine whether it is an induced subgraph of a grid (and also to produce its vertices' coordinates in a grid - see \cite{GSZ23} and references therein).

\begin{corollary}
    \textsc{Partial Domination}(Grids) is NP-complete.
\end{corollary}

We now turn to the other graph class of interest to us - the hypercubes $\mathcal{Q}$.



\begin{theorem}[Abbott and Katchalski \cite{AK91,AK88}]\label{thm:ak-snake}
    For any $d\ge 2$, the hypercube $Q_d$ contains an induced path on $\frac{77}{256}2^d$ vertices. Given $d$, the coordinates of such a path may be produced in time polynomial in $2^d$.
\end{theorem}

In their work, Abbott and Katchalski state there is an induced cycle on \textbf{strictly more than} $\frac{77}{256}2^d$ vertices, which entails an induced path on exactly $\frac{77}{256}2^d$ vertices.
The authors do not explicitly address the runtime of their construction in their work. However, it is clear from their proof that their description of the induced cycle can be realized as a recursive algorithm with such a runtime. 



\begin{corollary}\label{cor:grid-in-hypercube}
    For any $d \ge 2$, the hypercube $Q_{2d}$ contains an induced grid on $(\frac{77}{256}2^d)^2$ vertices. Given $d$, the coordinates of such a grid may be produced in time polynomial in $2^d$.
\end{corollary}

\begin{proof}
    Given $d$, produce coordinates of a path $P=\{p_1, p_2, \ldots, p_\ell\}$ of length $\ell=\frac{77}{256}2^d$ in $Q_d$ by applying Theorem \ref{thm:ak-snake}. Note that each $p_i$ is a bitstring of length $d$ exactly. Then the set $\{p_ip_j : i,j \in [\ell]\}$ is an induced grid of size $(\frac{77}{256}2^d)^2$ in $Q_{2d}$, and the result follows.
\end{proof}


\begin{theorem}\label{thm:hypercube-partial-domination-np-c}
    \textsc{Partial Domination}($\mathcal{Q}$) is NP-complete.
\end{theorem}

\begin{proof}
    Let $(G,T,k)$ be an instance of \textsc{Partial Domination}(Grids). We assume without loss of generality that $G$ is an $n \times n$ grid (if necessary, by extending $G$ in some dimension and retaining the same set $T$).
    We shall denote each vertex in $G$ by $v_{i,j}$ with $i,j \in [n]$. 
    Let $d=\lceil \log_2(\frac{256n}{77})\rceil$. Applying Corollary \ref{cor:grid-in-hypercube}, we may efficiently produce a mapping from $V(G)$ (vertices of the $n \times n$ grid) to $V(Q_{2d})$. Denote this mapping $f$.
    Let $G'=Q_{2d}$, and $T'=\{f(t) : t \in T\}$. 
    Then $G'[T']=G[T]$ (so $\gamma(G'[T'])=\gamma(G[T])$ also) and $(G',T',k)$ is an instance of \textsc{Partial Domination}($\mathcal{Q}$). The construction of $G'$ and $T'$ is feasible in polynomial time, and the result follows. \qed
\end{proof}


\subsection{Lunar graph classes}

\begin{definition}[Moon, Planet, Sun]
    We say a graph $G$ is the \emph{moon} in some graph $H$ if:
    \begin{itemize}
        \item There is some set $M\subset V(H)$ with $H[M]=G$. We also call $M$ the \emph{moon} in $H$.
        \item There is some $o \in V(H)$ and integer $r$ such that the set $\surface:=S(o,r)$ is a sphere of cardinality at least $|M|$ and $\planet:=B(o,r)$ is the ball with the same center and radius. We call $\planet$ the \emph{planet} and $\surface$ the \emph{planet surface} (or, briefly, \emph{surface}) in $H$.
        \item $N[M] \cap N[\planet]=\emptyset$ (the planet and the moon are far apart).
        \item $|\surface| \ge |M|$ (the surface is bigger than the moon).
        \item There is some set $S \subset V(H)$ (the \emph{sun} in $H$) such that $|S| \ge |N[\planet]| + |N[M]|$ (the sun is bigger than the moon and planet together) and $N[S]$ is disjoint from $N[\planet]$ (the sun and planet are far apart). Moreover any node in $S$ is at distance at least $2r$ from any node in $M$ (the sun and moon are very far apart).
    \end{itemize}
\end{definition}


\begin{definition}[lunar graph class.]
    We say a graph class $\mathcal{L}$ is \emph{lunar} in a graph class $\mathcal{H}$ if, for each $G \in \mathcal{L}$, there exists some $H \in \mathcal{H}$ such that $G$ is the moon in $H$. 
    We further require that such a graph $H$ (and vertex sets $M,\surface,S$ within it) can be constructed in polynomial time from $G$ (which entails that $H$ is at most polynomially larger than $G$). We say a graph class $\mathcal{L}$ is \emph{lunar in itself} (or simply \emph{lunar}) if the above holds for $\mathcal{H}=\mathcal{L}$.
\end{definition}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\linewidth,page=10]{RRP_algowin_figs.pdf}
    \caption{Illustration of our construction where $n=5, m=3, r=4$. The $28 \times 11$ grid contains the $5 \times 3$ grid as a moon. 
    Marked are: the moon $M$ (square vertices); $o=(n+r,m+r)=(7,9)$, together with the planet $\planet=B(o,r)$ ($o$ and disk and circle vertices) and its surface $\surface=S(o,r)$ (circle vertices); the sun $S=\{(i,j) : i \le 8\}$ (cross vertices).}
    \label{fig:lunar-grids}
\end{figure}

\begin{lemma}\label{cor:grids-are-lunar}
    The class of grid graphs is lunar in itself.
\end{lemma}
\begin{proof}
    The reader may find the illustrative example in Figure \ref{fig:lunar-grids} helpful. Let $G$ be some $n \times m$ grid (w.l.o.g. $n \ge m$, so $|G|$ is polynomial in $n$). 

    We shall use the fact that a sphere of radius $r \ge 1$ in a grid (which does not spill over the grid's boundary) has size $4r$. 
    
    Let $r=\lceil \frac{nm}{4} \rceil$. 
    Let $x=2(n + 2r + 1)$, and let $y=2(m + 2r)$. We choose $H$ to be the $x \times y$ grid.
    Then we identify:
    \begin{itemize}
        \item The moon: $M=V(G)$ (vertices of the $n\times m$ grid are also vertices of $x \times y$ grid).
        \item The planet: $o=(n+r, m+r)$, $\surface=S(o,r)$, $\planet=B(o,r)$. 
        \item The sun: $S=\{(i,j) : i \ge n + 2r + 3\}$.
    \end{itemize}
    It is easy to verify that the neighborhoods of the moon, planet and sun are disjoint; that the sun and moon are at distance at least $2r$; that the size of the planet exceeds that of the moon; and that the size of the sun exceeds that of the moon and planet's neighborhoods combined. Since our construction may be carried out in polynomial time, the result follows.
\end{proof}

The $x \times y$ grid is an induced subgraph of the $2x \times 2y$ toroidal grid, with the notable property that every shortest path in the former remains a shortest path in the latter. Applying this fact, the proof above can straightforwardly be adapted to obtain the following corollary:

\begin{corollary}\label{cor:torus-grids-are-lunar}
    The class of grid graphs is lunar in the class of toroidal grid graphs.
\end{corollary}


\begin{lemma}\label{lem:hypercubes-are-lunar}
    The class of hypercubes $\mathcal{Q}$ is lunar in itself.
\end{lemma}

\begin{proof}    
    Note that we reuse some of the notation from our proof of Theorem \red{[hypercube rrp]}.
    Let $G\in \mathcal{Q}$ be some hypercube of dimension $d$, i.e. $G=Q_d$ for some $d$. We define:
    \begin{itemize}
        \item Let $\ell=6d+9$ and $H=Q_{\ell}$.
        \item Let $M:=\{0^{5d+9}x : x \in Q_d\}$. 
        \item Let $o:=0^{4d+6}1^{2d+3}$ and $r=d$. Recall we denote the planet $\planet=B(o,r)$ and its surface  $\surface=S(o,r)$. 
        \item Let $S:=\{\overline{x} : x \in N[\planet] \cup N[M]\}$. Intuitively, the sun nodes are the reflection of the neighborhoods of planet nodes and moon nodes.
        
    \end{itemize}

    The illustration in Figure \ref{fig:lunar-hypercube-weights} will be helpful in verifying the following:
    \begin{itemize}
        \item $H[M]=G$.
        \item The sphere $\surface=S(o,r)$ has cardinality at least $|Q_d|$ (easy to see by considering $\{o \oplus 0^{4d+9}\overline{x}{x} : x \in Q_d\}$, which clearly contains only vertices at distance exactly $d$ from $o$ and so is a subset of $\surface$).
        \item $N[M]$ and $N[\planet]$ are disjoint. 
        \item $N[M]$ and $N[\planet]$ contain only vertices with at most $3d+4$ ones. 
        \item $|S| \ge |N[\planet]| + |N[M]|$ (by applying both two points above).
        \item $N[S]$ is disjoint from $N[M]$ and $N[\planet]$.
        \item Moreover any node in $S$ is at distance at least $2r$ from any node in $M$. 
    \end{itemize}

    Note that $Q_\ell$ has size $2^{6d+9}=2^9\cdot (2^d)^6$ which is polynomial in the size of $Q_d$. The result follows.
    \qed
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth, page=9]{RRP_algowin_figs.pdf}
    \caption{Illustration of our proof hypercubes are lunar, showing the weights (number of ones in any vertex label) for different sets of vertices. The midsection of the hypercube (separating majority-1 vertices from majority-0 vertices) is shown as a dashed line.}
    \label{fig:lunar-hypercube-weights}
\end{figure}



\subsection{The main result}

We are now able to state and prove the main result of this section.

\begin{theorem}\label{thm:hypercubeRRPsigma2}
    For any fixed $\mu \in (0,1)$, and any graph classes $\mathcal{L}$ and $\mathcal{G}$ with $\mathcal{L}$ lunar in $\mathcal{G}$, the problem \textsc{Partial Domination}($\mathcal{L}$) is polynomially reducible to the problem \textsc{1-switched RRP($\delta = 1$)} restricted to instances $(H, \mu, D, \kappa)$ satisfying:
	\begin{itemize}
		\item $H\in \mathcal{G}$, and 
		\item the workload matrix $D$ is sparse and all values in it are polynomial in $|H|$.
	\end{itemize}
\end{theorem}

\begin{proof}
    We are given an instance $(G, T, k)$ of \textsc{Partial Domination}($\mathcal{L}$), with $G\in \mathcal{L}$, a set of vertices $T \subseteq V(G)$, and integer $k$. We shall produce an instance $(H, \mu, D, \kappa)$ of \textsc{1-Switched RRP}($\delta=1$).
    $\mu$ is some prescribed value between $0$ and $1$, as in the theorem statement.
    
    The graph $H$, along with vertex sets $M,\surface,\planet,S$, the vertex $o$, and the integer $r$, are obtained by applying the definition of a lunar class. We denote by $T'$ the set of vertices in $H$ to which $T$ is mapped, so that $H[M][T]=H[T']=G[T]$.

    In order to describe our demands $D$, we identify some useful sets of vertices in $H$:
    \begin{itemize}
        \item \emph{Target vertices} are exactly the set $T'=\{t_1',t_2',\ldots, t_{|T|}'\}$. 
        \item The set of moonlit nodes $\moonlit=\{\breve{m}_1,\breve{m}_2,\ldots,\breve{m}_k\}$ is some arbitrary subset of $\surface$ with cardinality $k$ exactly.
        \item The set of sunlit nodes $\sunlit:= N[M] \cup N[\planet] \setminus (T \cup \moonlit)$. 
    \end{itemize}

    The intention is that our construction will ensure that, in any configuration $N$ of interest to us, the moonlit nodes $\moonlit$ (resp. sunlit nodes $\sunlit$) will be connected by a dynamic link to moon nodes $M$ (resp. sun nodes $S$). 
    
    Consider a new graph: the complete bipartite graph with $\sunlit \cup S$ as vertices and $\sunlit \times S$ as edges. Let $E_S$ be an arbitrary maximum matching in this bipartite graph. Note that $|S| \ge |\sunlit|$ by construction, and so $|E_S|=|\sunlit|$ exactly and each sunlit vertex is incident to exactly one edge in $E_S$. Note that by construction $E_S \cap E(H) = \emptyset$, because none of the sunlit nodes are adjacent to any sun node (by applying a property of lunar graphs). That is, if $(u,v)$ is an edge in $E_S$ then $u$ and $v$ are not adjacent in $H$. 
    
    Let $\alpha=(r+\mu+1)|T|$. Our demand matrix $D$ is fully described by the following: 
    \begin{itemize}
        \item $D[u,v]=\alpha$ for each $(u,v)\in E_S$ (sunlight demands), 
        \item $D[o,t]=1$ for each $t\in T$ (moonlight demands), and
        \item all other entries of $D$ are zero.
    \end{itemize}
    
    \begin{figure}
        \centering
        \includegraphics[width=0.8\linewidth, page=8]{RRP_algowin_figs.pdf}
        \caption{Illustration of the demands described in our reduction, for the instance $(G,T,4)$ of \textsc{Partial Domination}(Grid graphs). Nodes of $T$ (and $T'$ in $H$) are shown as black squares; other nodes of $G$ (and $M$ in $H$) are shown as boxes. Other nodes are shown as in Figure \ref{fig:lunar-grids} earlier.
        Moonlight demands are shown as solid blue curves. The sunlit nodes $\sunlit$ are those in orange shaded regions (note exactly $4$ nodes of $\surface$ are not sunlit - these are the moonlit nodes $\moonlit$). Sunlit demands are drawn as orange arcs (for clarity, only a few are shown).}
        \label{fig:lunar-construction-demands}
    \end{figure}
    

    It remains for us to define $\kappa$. As before, we define this as $\kappa_\alpha + \kappa_1$, with $\kappa_\alpha = \mu \alpha |E_S|$, and $\kappa_1 = |T|(r + \mu) + |T| - k$. We note that $\alpha > \kappa_1$.
    This completes our construction of the instance $(H, \mu, D, \kappa)$.

    \begin{claim}
        If $(G,T,k)$ is a yes-instance of \textsc{Partial Domination} then $(H, \mu, D, \kappa)$ is a yes-instance of \textsc{1-Switched RRP}($\delta=1$).
    \end{claim}
    \begin{proof}
        An illustration of an optimal configuration is shown in Fig. \ref{fig:optimal-lunar-configuration}.
        Let $X$ be a dominating set of $G[T]$ of cardinality $k$. Denote also by $X'=\{x_1',x_2', \ldots, x_k'\}$ the corresponding set of vertices in $H$. 
        
        Let $N := E_S \cup \{(x_i', \breve{m}_i) : 1 \le i \le k\}$. Clearly, under $N$ each sunlight demand is served at cost exactly $\mu \alpha$ and so all sunlight demands cumulatively are served at cost $|E_S|\mu\alpha=\kappa_\alpha$. 

        Further, the $k$ demands from each node $x_i'$ to $o$ are each served at cost exactly $\mu+r$ (by the path $x_i'\dynamic \breve{m}_i \rightsquigarrow_{r} o$), and the moonlit demand for each of the $|T|-k$ other nodes $t\in T$ is served at cost exactly $1 + \mu + r$ (by the path $t \rightsquigarrow_1 x_i' \dynamic \breve{m}_i \rightsquigarrow_{r} o$). The claim follows.\qed
    \end{proof}

    \begin{figure}[!ht]
        \centering
        \includegraphics[width=0.6\linewidth, page=11]{RRP_algowin_figs.pdf}
        \caption{Detail of an optimal configuration $N$for the instance shown in \ref{fig:lunar-construction-demands}. Only moonlight demands (solid blue arcs) and dynamic links serving them (dashed red lines) are shown. Note that all moonlit demands are served at cost exactly $\kappa_1$.}
        \label{fig:optimal-lunar-configuration}
    \end{figure}
    

    Conversely, suppose that $(H, \mu,D,\kappa)$ is a yes-instance of \textsc{1-switched RRP($\delta=1$)} and that $N$ is a configuration and $F$ a set of flow-paths witnessing that the total workload cost is at most $\kappa$. 
	
	\begin{claim}\label{clm:all-sunlit}
        Each sunlit node has a line of sight (optic link) to a sun node.	
        Formally, every edge $(u,v)$ of $E_S$ is necessarily such that $(u,v)\in N$ and the total workload cost of flow-paths serving the $\alpha$-demands is exactly $\kappa_\alpha$.        
	\end{claim}

    \begin{proof}
    	Suppose that at least one of the $\alpha$-demands is served via a flow-path at a workload cost of more than $\mu\alpha$; so, it must be at a workload cost of more than $(1+\mu)\alpha$ as we cannot traverse a dynamic link followed immediately by another dynamic link (recall, $\Delta_S=1$) and by our construction, if $D[u,v]=\alpha$ then there is no static link $(u,v)$. Hence, the total workload cost of flow-paths serving the $\alpha$-demands is at least $(|E_\alpha| - 1)\mu\alpha + (1+\mu)\alpha = \kappa_\alpha +\alpha$. We have that $\kappa_1 < (r+\mu+1)|T| = \alpha$. Hence, the total workload cost of all flow-paths of $F$ is strictly greater than $\kappa$ which yields a contradiction and the claim follows.
    \qed \end{proof}

    \begin{claim}\label{clm:moonlit-demands}
        Each moonlight demand is served at cost at least $\mu + r$. Furthermore, at most $k$ moonlight demands are served at cost $\mu + r$ exactly. 
    \end{claim}
    \begin{proof}
        Consider some moonlight demand; necessarily it has form $D[t,o]=1$ for some $t\in T$.
        
        We first show each moonlight demand is served at cost at least $\mu+r$. Suppose for contradiction that $D[t,o]$ is served at cost strictly less than $\mu + r$. Since $t$ and $o$ are at distance at least $r+3$, the flow-path from $t$ to $o$ must make use of some dynamic link $u \dynamic v$ at cost $\mu$. The static portion of the path therefore must have cost at most $r-1$, which entails that $v \in B(o,r-1) \subsetneq \sunlit$ (that is, $v$ is a sunlit node). Applying Claim \ref{clm:all-sunlit} $v$ is connected by dynamic link to some sun node, so $u \in S$ necessarily. Then the path from $t$ to $u$ has length at least $2r$, yielding the desired contradiction. 

        Now observe that $D[t,o]$ can be served at cost exactly $\mu + r$ if and only if the dynamic link $t \dynamic \breve{m}$ exists, for some $\breve{m} \in \moonlit$. Since $|\moonlit|=k$ exactly by construction, we obtain that this may be the case for at most $k$ nodes in $T$. The claim follows. 
        \qed
    \end{proof}

    
    Since $\kappa_1 = (r+\mu)(k) + (r + \mu + 1)(|T|-k)$, we immediately obtain that \emph{exactly} $k$ moonlight demands are served at cost $r+\mu$ and all remaining moonlight demands are served at cost $r+\mu+1$ exactly.
        
    \begin{claim}\label{clm:all-moonlit}
        The set $X=\{ u: (u,v)\in N $ and $v\in \breve{M}$ is a moonlit node$\}$ is a dominating set of $H[M]$.
    \end{claim}
    \begin{proof}
        Suppose for contradiction that there is some vertex $t\in T'$ which is neither in $X$ nor adjacent to any vertex in $X$. We show that the cost of serving the demand $D[y,o]=1$ is strictly greater than $r + \mu + 2$. Denoting arbitrary nodes $m'\in N[M],\planetv' \in N[\planet], \surfacev \in \surface$, this flow is routed either:
        \begin{itemize}
            \item Via static links only, along a path of length at least $r+3>r+\mu+1$:
            $y\rightsquigarrow_{\ge1} m' \rightsquigarrow_{\ge1} \planetv' \rightsquigarrow_1 \surfacev \rightsquigarrow_r o$, or
            \item Via static links and one dynamic link $u\dynamic v$ with:
            \begin{itemize}
                \item $v$ in $\surface$, at cost at least $r+\mu+2>r+\mu+1$: 
                $y \rightsquigarrow_{\ge 2} u \dynamic v \rightsquigarrow_r o$
                \item $u$ and $v$ both outside $N[\planet]$, at cost at least $r+\mu+2>r+\mu+1$: 
                $y \rightsquigarrow_{\ge 0} u \dynamic v \rightsquigarrow_{\ge 1} \planetv' \rightsquigarrow_1 \surfacev \rightsquigarrow_r o$
                \item either $u$ or $v$ in $N[\planet] \setminus \surface$ (and the other in $S$), at cost at least $2r + \mu$ (recall all vertices in $S$ are distance at least $2r$ from any vertex in $M$).
            \end{itemize}
        \end{itemize}
        This contradicts our earlier claim (that all moonlight demands are served at cost at most $r+\mu+1$) and the result follows.\qed
    \end{proof}
    We note that the construction described takes polynomial time, and the main result follows.
\qed    
\end{proof}

Applying our earlier results on lunar graph classes (Lemmas \ref{lem:hypercubes-are-lunar} and \ref{lem:grids-are-lunar}, Corollary \ref{cor:torus-grids-are-lunar}) together with Theorem \ref{thm:hypercube-partial-domination-np-c} we obtain that RRP remains hard even when the number of dynamic links admitted on any path is limited to $1$.

\begin{corollary}
    \textsc{1-switched RRP($\delta = 1$)($\mathcal{G}$)} is NP-complete if $\mathcal{G}$ is: the class of hypercubes;  the class of grid graphs; or the class of toroidal grid graphs.
\end{corollary}

We emphasize again the value of hypercubes as a prototypical model of interconnection networks, and additionally note that grids and toroidal grids exhibit additional properties which may have been expected to yield a tractable setting, such as planarity and bounded degree. 
The restriction to $\delta=1$ in our setting also implies a restriction to $\sigma=2$ (as 3 alternations along a path would entail a minimum 2 dynamic links along the same) but the converse does not hold; we expect that the case of \textsc{1-Switched RRP}($\sigma=2, \delta=2$) can be shown to be intractable through similar proof techniques, but leave this for future work.
